Automated crater shape retrieval using weakly-supervised deep learning

Crater ellipticity determination is a complex and time consuming task that so far has evaded successful automation. We train a state of the art computer vision algorithm to identify craters in Lunar digital elevation maps and retrieve their sizes and 2D shapes. The computational backbone of the model is MaskRCNN, an "instance segmentation" general framework that detects craters in an image while simultaneously producing a mask for each crater that traces its outer rim. Our post-processing pipeline then finds the closest fitting ellipse to these masks, allowing us to retrieve the crater ellipticities. Our model is able to correctly identify 87\% of known craters in the longitude range we hid from the network during training and validation (test set), while predicting thousands of additional craters not present in our training data. Manual validation of a subset of these "new" craters indicates that a majority of them are real, which we take as an indicator of the strength of our model in learning to identify craters, despite incomplete training data. The crater size, ellipticity, and depth distributions predicted by our model are consistent with human-generated results. The model allows us to perform a large scale search for differences in crater diameter and shape distributions between the lunar highlands and maria, and we exclude any such differences with a high statistical significance. The predicted test set catalogue and trained model are available here: https://github.com/malidib/Craters_MaskRCNN/.

==> oldbibliography <==
\begin{thebibliography}{00}

\bibitem{1} Emami E., Bebis G., Nefian A., Fong T. (2015) Automatic Crater Detection Using Convex Grouping and Convolutional Neural Networks. In: Bebis G. et al. (eds) Advances in Visual Computing. Lecture Notes in Computer Science, vol 9475. Springer, Cham

\bibitem{2} Stepinski, T. F., Wei Ding, and R. Vilalta. "Detecting impact craters in planetary images using machine learning." Intelligent Data Analysis for Real-Life Applications: Theory and Practice, IGI Global (2012): 146-159.

\bibitem{3} Salamuni{\'c}car, G., \& Lon{\v c}ari{\'c}, S.\ 2010.\ Method for crater detection from martian digital topography data using gradient value/orientation, morphometry, vote analysis, slip tuning, and calibration.\ IEEE Transactions on Geoscience and Remote Sensing 48, 2317-2329.

\bibitem{4} Wetzler, P., Honda, R., Enke, B., Merline, W., Chapman, C., \& Burl, M. (2005). Learning to detect small impact craters. Seventh IEEE Workshops on Application of Computer Vision., 1, pp. 178-184. Breckenridge.

\bibitem{5} Cohen, J.P., Lo, H.Z., Lu, T., Ding, W., 2016. Crater Detection via Convolutional Neural
Networks. In: Proceedings of the 47th Lunar and Planetary Science Conference,
Abstract \# 1143.

\bibitem{6} Palafox, Leon F., et al. "Automated detection of geological landforms on Mars using Convolutional Neural Networks." Computers \& Geosciences 101 (2017): 48-56.

\bibitem{7} Bandeira, Louren�o, Wei Ding, and Tomasz F. Stepinski. "Detection of sub-kilometer craters in high resolution planetary images using shape and texture features." Advances in Space Research 49.1 (2012): 64-74.

\bibitem{8} Zhang, Yingying, et al. "Single-image crowd counting via multi-column convolutional neural network." Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition. 2016.

\bibitem{9} Zeng, Lingke, et al. "Multi-scale Convolutional Neural Networks for Crowd Counting." arXiv preprint arXiv:1702.02359 (2017).

\bibitem{10} Krizhevsky, Alex, Ilya Sutskever, and Geoffrey E. Hinton. "Imagenet classification with deep convolutional neural networks." Advances in neural information processing systems. 2012.

\bibitem{11} Ciregan, Dan, Ueli Meier, and J�rgen Schmidhuber. "Multi-column deep neural networks for image classification." Computer Vision and Pattern Recognition (CVPR), 2012 IEEE Conference on. IEEE, 2012.

\bibitem{12} Long, Jonathan, Evan Shelhamer, and Trevor Darrell. "Fully convolutional networks for semantic segmentation." Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition. 2015.

\bibitem{13} Ronneberger, Olaf, Philipp Fischer, and Thomas Brox. "U-net: Convolutional networks for biomedical image segmentation." International Conference on Medical Image Computing and Computer-Assisted Intervention. Springer, Cham, 2015.

\bibitem{14} LeCun, Yann, et al. "Backpropagation applied to handwritten zip code recognition." Neural computation 1.4 (1989): 541-551.

\bibitem{15} Kingma, Diederik, and Jimmy Ba. "Adam: A method for stochastic optimization." arXiv preprint arXiv:1412.6980 (2014).

\bibitem{16} Srivastava, Nitish, et al. "Dropout: a simple way to prevent neural networks from overfitting." Journal of machine learning research 15.1 (2014): 1929-1958.

\bibitem{17} Greeley, Ronald, and Donald E. Gault. "Precision size-frequency distributions of craters for 12 selected areas of the lunar surface." Earth, Moon, and Planets 2.1 (1970): 10-77.

\bibitem{18} Kirchoff, M., K. Sherman, and C. Chapman. "Examining lunar impactor population and evolution: Additional results from crater distributions on diverse terrains." EPSC-DPS Joint Meeting 2011. 2011.

\bibitem{19} Robbins, Stuart J., et al. "The variability of crater identification among expert and community crater analysts." Icarus 234 (2014): 109-131.

\bibitem{20} Abadi, Mart�n, et al. "Tensorflow: Large-scale machine learning on heterogeneous distributed systems." arXiv preprint arXiv:1603.04467 (2016).

\bibitem{21} Chollet, Fran\c{c}ois et al. "Keras." Github (2015) \url{https://github.com/fchollet/keras}

\bibitem{22} Van der Walt, Stefan, et al. "scikit-image: image processing in Python." PeerJ 2 (2014): e453.

\bibitem{23} Yu, Fisher, and Koltun, Vladlen. "Multi-Scale Context Aggregation by Dilated Convolutions". Computing Research Repository, arXiv preprint arXiv:1511.07122 (2015). 

\bibitem{24} Abadi, Martín, et al. "Tensorflow: Large-scale machine learning on heterogeneous distributed systems." arXiv preprint arXiv:1603.04467 (2016).

\bibitem{25} Gal, Yarin, and Zoubin Ghahramani. "Dropout as a Bayesian approximation: Representing model uncertainty in deep learning." international conference on machine learning. 2016.

\bibitem[Di et al.(2014)]{dili} Di, K., Li, W., Yue, Z., Sun, Y., Liu, Y.\ 2014.\ A machine learning approach to crater detection from topographic data.\ Advances in Space Research 54, 2419-2429. 


\bibitem[Chung et al.(2014)]{chungchung} Chung, C. P., Chung, O. C., Yam, C. H.\ 2014.\ Lunar Crater Identification from Machine Learning Perspective.\ Acta Futura 9 (2014) 41-45.


\bibitem[Thorey(2015)]{thorey} Thorey, C.\ 2015.\ Detection of lunar floor-fractured craters using machine learning methods.\ European Planetary Science Congress 2015, id.EPSC2015-95 10. 

\bibitem[Boukercha et al.(2014)]{boukercha} Boukercha, A., Al-Tameemi, A., Grumpe, A., W{\"o}hler, C.\ 2014.\ Automatic Crater Recognition Using Machine Learning with Different Features and Their Combination.\ Lunar and Planetary Science Conference 45, 2842. 

\bibitem[Simonyan and Zisserman(2014)]{simon} Simonyan, K., Zisserman, A.\ 2014.\ Very Deep Convolutional Networks for Large-Scale Image Recognition.\ ArXiv e-prints arXiv:1409.1556. 

\bibitem[Szegedy et al.(2014)]{gedy} Szegedy, C., Liu, W., Jia, Y., Sermanet, P., Reed, S., Anguelov, D., Erhan, D., Vanhoucke, V., Rabinovich, A.\ 2014.\ Going Deeper with Convolutions.\ ArXiv e-prints arXiv:1409.4842. 

\bibitem[Gomes et al.(2005)]{n1} Gomes, R., Levison, H.~F., Tsiganis, K., Morbidelli, A.\ 2005.\ Origin of the cataclysmic Late Heavy Bombardment period of the terrestrial planets.\ Nature 435, 466-469. 


\bibitem[Morbidelli et al.(2005)]{n2} Morbidelli, A., Levison, H.~F., Tsiganis, K., Gomes, R.\ 2005.\ Chaotic capture of Jupiter's Trojan asteroids in the early Solar System.\ Nature 435, 462-465. 


\bibitem[Tsiganis et al.(2005)]{n3} Tsiganis, K., Gomes, R., Morbidelli, A., Levison, H.~F.\ 2005.\ Origin of the orbital architecture of the giant planets of the Solar System.\ Nature 435, 459-461. 

\bibitem[Salamuni{\'c}car et al.(2014)]{sala+14} Salamuni{\'c}car, G., Lon{\v c}ari{\'c}, S., Grumpe, A., \& W{\"o}hler, C.\ 2014.\ Hybrid method for crater detection based on topography reconstruction from optical images and the new LU78287GT catalogue of Lunar impact craters.\ Advances in Space Research, 53, 1783-1797.

\bibitem[Met Office (2015)]{cartopy} Met Office. "Cartopy: a cartographic python library with a matplotlib interface." SciTools (2015) \url{http://scitools.org.uk/cartopy/}

\bibitem[LOLA Science Team (2014)]{lola14}LOLA Science Team.\ "LRO LOLA Elevation Model 118m (LDEM GDR)."  USGS Astrogeology Science Center (2014) \url{https://astrogeology.usgs.gov/search/details/Moon/LRO/LOLA/Lunar_LRO_LOLA_Global_LDEM_118m_Mar2014/cub}

\end{thebibliography}
